Gradient-free Online Learning in Games with Delayed Rewards

Motivated by applications to online advertising and recommender systems, we consider a game-theoretic model with delayed rewards and asynchronous, payoff-based feedback. In contrast to previous work on delayed multi-armed bandits, we focus on multi-player games with continuous action spaces, and we examine the long-run behavior of strategic agents that follow a no-regret learning policy (but are otherwise oblivious to the game being played, the objectives of their opponents, etc.). To account for the lack of a consistent stream of information (for instance, rewards can arrive out of order, with an a priori unbounded delay, etc.), we introduce a gradient-free learning policy where payoff information is placed in a priority queue as it arrives. In this general context, we derive new bounds for the agents' regret; furthermore, under a standard diagonal concavity assumption, we show that the induced sequence of play converges to Nash equilibrium with probability $1$, even if the delay between choosing an action and receiving the corresponding reward is unbounded.

==> Algorithms/ODP.tex <==
%----------------------------------------------------------------------
%%% ODP FRAMEWORK
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\tt
\small
\setstretch{1.05}
\begin{algorithmic}[1]
\For{$\run=\running$}
	\State	
		draw $\unitvar_{\run}$ uniformly from $\sphere^{\vdim}$
		\Comment{perturbation direction}%
	\State
		set $\pertvar_{\run}\leftarrow\unitvar_{\run} - (\state_{\run} - \base)/\radius$
		\Comment{feasibility adjustment}%
	\State
		play $\est\state_{\run} \leftarrow \state_{\run} + \mix_{\run} \pertvar_{\run}$
		\Comment{player chooses action}%
	\State
		generate payoff $\pay_{\run} = \pay(\est\state_{\run})$
		\Comment{associated payoff}%
	\State
		trigger delay $\delay_{\run}$
		\Comment{delay for payoff}%
	\State
		collect rewards $\info_{\run} = \setdef{\runalt}{\runalt + \delay_{\runalt} = \run}$
%		reap $\reward_{\run} = \sum_{\runalt\in\info_{\run}} \pay_{\runalt}$
		\Comment{receive past payoffs}%
%	\State
%		get reward $\reward_{\run} = \sum_{\runalt\in\info_{\run}} \pay_{\run}$
%		\Comment{receive payoff feedback}%
	\State
		update pipeline $\pool_{\run} \leftarrow \pool_{\run-1} \cup \info_{\run}$
		\Comment{enqueue received info}%
	\State
		take $\head_{\run} = \min \pool_{\run}$;
		set $\pool_{\run} \leftarrow \pool_{\run}\exclude{\head_{\run}}$
		\Comment{dequeue oldest info}
	\State
		set $\est\payv_{\run}\leftarrow (\vdim/\mix_{\head_{\run}}) \pay_{\head_{\run}} \, \unitvar_{\head_{\run}}$
		\Comment{estimate gradient}%
	\State
		update $\state_{\run+1} \leftarrow \Eucl(\state_{\run} + \step_{\run} \est\payv_{\run})$
		\Comment{update pivot}%
\EndFor
\end{algorithmic}

==> App-Proofs.tex <==
%----------------------------------------------------------------------
%%% APP: PROOFS
%----------------------------------------------------------------------
% !TEX root = ./Supplement.tex

\section{Properties of the pooling strategy}

In this section we prove some key properties of the information queueing/dequeing strategy that is a crucial element of the \ac{GOLD} algorithm.
This strategy allows the players to receive rewards and thus to update their strategies often (see \cref{lem:noupdate}), while ensuring that rewards do not stay too long in the pool (\ref{lem:delayedfeedback}).
We also show that the delay rate allows us to ensure convergence properties needed for the proof of \cref{thm:main}.


\begin{lemma}
\label{lemma:noupdate}
The maximal number of steps with an empty pool \textpar{no update} is bounded by the maximal delay so far, \ie
\begin{equation}
\#\setdef{\runalt}{\pool_\runalt=\varnothing, \runalt=\running\run}
	\leq \max\nolimits_{1\leq \runalt \leq\run} (\delay_\runalt).
\end{equation}
\end{lemma}

\begin{proof}
We begin by analyzing the \emph{constant delay} case, \ie when $\delay_\runalt=\Delay$ for all $\runalt=\running\run$.
In that case, the first $\Delay$ steps have no update;
subsequently, at each stage, the agent receives payoff information with delay $\Delay$.

Now assume that $(\delay_\run)_{\run=\running\run}$ is a sequence of delays.
We prove that if we modify the sequence by $\delay'_\runalt<\delay_\runalt$, the number of steps without an update will remain the same or decrease by one.
Indeed, the reward of the $\runalt$-th was collected in step $\delay_\runalt+ \runalt$ and is now collected in step $\delay'_\runalt+ \runalt$.
This will increase the size of the pool, $\pool_{\delay'_\runalt+ \runalt}$ by 1, and will allow to provide an update to the next step without update (it could be $\delay'_\runalt+ \runalt$).
If the next step without update was before $\run$, the number of steps without update decreases by one, otherwise it stays the same (\cref{fig:delay_change} provides a graphical illustration of the argument).

%\begin{figure}[!h]
 %    \center{ \includegraphics[width=.9\linewidth]{Figures/delay_s.pdf}}
   % \caption{Evolution of the number of steps without an update if we change $\delay_\runalt$ by $\delay'_\runalt<\delay_\runalt$. Two cases are presented, above, there was no step without update between $\delay'_\runalt + \runalt$ and $\delay_\runalt+ \runalt$, so the number of steps without update does not change. Below there is a step without update between $\delay'_\runalt + \runalt$ and $\delay_\runalt+ \runalt$, after the change (red) this step has an update, but a step after $\delay_\runalt+ \runalt$ loses its update.}
   %\label{fig:b_and_c}
%\end{figure}


\begin{figure}[!h]
\begin{center}
\input{Figures/DelaySchematics.tex}
\end{center}


\begin{center}
\input{Figures/DelaySchematics_bis.tex}
\end{center}
    \caption{Evolution of the number of steps without an update if we reduce a delay. The case presented is when the number of steps without update decreases. Here the delay of step $1$ decreases from $3$ to $1$, as a consequence, step $3$ has an update that it previously did not have.}
   \label{fig:delay_change}
\end{figure}

This means that the maximal number of steps without update is reached when the delay is constant and is equal to said delay.
Our claim then follows immediately.
\end{proof}


We proceed to bound the difference between the time an information is used and the time it was generated:

\begin{lemma}
\label{lemma:delayedfeedback}
The difference $\run-\head_{\run}$ between the step when a reward is observed and the step when the action was taken is bounded from above by the maximal delay up to step $\run$.
\end{lemma}

\begin{proof}
We proceed by induction.
Since at first the pool is empty, one of the rewards arriving in the first non-empty $\info$ is used, so $\run-\head_{\run}=\delay_{\head_{\run}}\leq \max\limits_{\runalt \leq \run} (\delay_{\runalt})$ in this case.

For the inductive step, assume that, until $\run \in \N$ we have $\run - \head_{\run} \leq \max\limits_{\runalt \leq \run} (\delay_{\runalt})$;
we prove below that this is also the case for $\run +1$.
In that case, $\pool_{\run+1} \leftarrow \pool_{\run} \cup \info_{\run+1}$ and $\head_{\run+1} = \min(\pool_{\run+1})$ so $ \min(\info_{\run+1})\geq \run +1 - \max\limits_{\runalt \leq \run +1} (\delay_{\runalt})$;
in addition, at the $\run$-th step, the oldest element of $\pool_{\run} $ is removed from the pool and utilized.
As a result, $ \min(\pool_{\run}) > \run - \max\limits_{\runalt \leq \run} (\delay_{\runalt})\geq \run +1 - \max\limits_{\runalt \leq \run +1} (\delay_{\runalt})$.
This gives $\head_{\run+1} \geq \run +1 - \max\limits_{\runalt \leq \run +1}( \delay_{\runalt})$ and completes the induction (and our proof).
\end{proof}

Our next lemma goes a step further by showing that, with high probability, the difference $\run-\head_{\run}$ is small relative to $\run$:

\begin{corollary}
\label{lemma:delay}
Under \cref{asm:delay}, we have $\run - \head_{\run} = o(\run^\alpha)$.
In particular, choosing $\alpha<1$, we get $\run-\head_{\run} = o(\run)$ and $\head_{\run}=\Theta(\run)$ .
\end{corollary}

\begin{proof}
This clearly comes from \cref{lemma:delayedfeedback} and \cref{asm:delay}.
\end{proof}

We proceed with a preparatory technical lemma establishing the convergence of certain series to a finite number of parameters that arise in the sequel:

%\begin{lemma*}
%\label{lem:3sums}
\textbf{Lemma} \ref{lem:3sums}
Suppose that \eqref{eq:GOLD} is run with step-size and sampling radius parameters of the form $\step_{\run} \propto \step/\run^{c}$ and $\mix_{\run} \propto \mix/\run^{b}$, with $b,c>0$.
Then:
\vspace{-\medskipamount}
\begin{enumerate}
\setlength{\itemsep}{0pt}
\item
If $2c-b \geq 1+\alpha$, then $\sum_{\run=\start}^{\nRuns} A_{t} = \bigoh(\log\nRuns)$;
in addition, if the inequality is strict, $A_{\run}$ is summable.
\item
If $c+b\geq 1$, then $\sum_{\run=\start}^{\nRuns} B_{t} = \bigoh(\log\nRuns)$;
in addition, if the inequality is strict, $B_{\run}$ is summable.
\item
If $2c - 2b \geq 1$, then $\sum_{\run=\start}^{\nRuns} C_{t} = \bigoh(\log\nRuns)$;
in addition, if the inequality is strict, $C_{\run}$ is summable.
\end{enumerate}
%\end{lemma*}

\begin{remark*}
For clarity, the conditions on $b$, $c$ and $\alpha$ are summarised in \cref{fig:b_and_c}.
\end{remark*}
 
\begin{proof}
We begin with the first series $\sum_{\runalt=\run}^\infty \step_{\runalt}\sum_{i=\head_{\runalt}}^{\runalt-1}\frac{\step_i}{\mix_i}$.
In this case, \cref{lemma:delay} gives us that, for large enough $\run$, we have $\runalt-\head_{\runalt}\leq A \runalt^\alpha \leq A \runalt $ $\forall \runalt>\run$ for a given $A$.
We also have that $1/\run^{b} \propto \mix_{\run} \leq \mix_{\head_{\run}} \propto 1/\head_{\run}^{b} = \Theta(1/\run^{b})$ so $\mix_{\head_{\run}} = \Theta(1/\run^{b})$.
In turn, this gives
\begin{align}
\step_{\runalt}\sum_{i=\head_{\runalt}}^{\runalt-1} \step_i/\mix_i
	\leq A\step_{\runalt} \runalt^\alpha \frac{\step_{\runalt}}{\mix_{\head_{\runalt}}}
%	\notag\\
%	&= \Theta(A\frac{1}{\runalt^c} \runalt^\alpha\frac{\runalt^{b}}{\runalt^c})
%	\notag\\
	= \Theta\parens*{\frac{1}{\runalt^{2c-\alpha-b}}},
\end{align}
so the condition $2c-b>1+\alpha$ is sufficient for convergence to a finite number and in the equality case we have $\sum_{\run=\start}^{\nRuns} A_{t} = \bigoh(\log\nRuns)$ as claimed.

\begin{figure}[htbp]
\centering
\input{Figures/b_c_a.tex}
\caption{The shaded region (green) indicates the possible choices of $b$ and $c$ given $\alpha$.}
\label{fig:b_and_c}
\end{figure}

For the second series, $ \sum_{\runalt=\run}^\infty\step_{\runalt}\mix_{\head_{\runalt}}$, note that $\step_{\runalt} \mix_{\head_{\runalt}} = \Theta(1/\runalt^{b+c})$, so the condition $c+b>1$ is sufficient for convergence to a finite number and in the equality case we have $\sum_{\run=\start}^{\nRuns} B_{t} = \bigoh(\log\nRuns)$.

Finally, for the last series, $\sum_{\runalt=\run}^\infty \step_{\runalt}^2 / \mix_{\head_{\runalt}}^2$, we have $\step_{\runalt}^2 / \mix_{\head_{\runalt}}^2 = \Theta(\runalt^{2b} / \runalt^{2c})$, so the condition $2c-2b>1$ is sufficient for convergence to a finite number and in the equality case we have $\sum_{\run=\start}^{\nRuns} C_{t} = \bigoh(\log\nRuns)$.
\end{proof}


\section{Regret minimization}
In this section we prove that the \ac{GOLD} policy leads to no regret under appropriate choices of the step-size and sampling radius sequences ($\step_{\run}$ and $\mix_{\run}$ respectively).
We start by proving the inequality of \cref{lem:dist}.

%\begin{theorem}
%\label{regret}
%Assume we have step size and sample radius such that $\step_{\run}=\Theta(\frac{1}{\run^c})$, $\mix_{\run}=\Theta(\frac{1}{\run^b})$ with $0<c<1$, $2c-2b>1$, and  $2c-b>1+\alpha$, $c+b>1$. We also assume that the delay is such that $\exof{\delay_{\run}^p}<\infty$ for $p>\frac{2}{\alpha}>2$.
%Then we can bound the expected regret of players playing Algorithm \ac{GOLD}  by $\max\limits_{\point \in \points}(\exof{\sum_{\runalt=1}^{\nRuns} (\pay(\point) -\pay(\state_\runalt))})=\bigoh(\nRuns^{\max(\frac{3}{4},\frac{2}{3}+\frac{\alpha}{3})})$.
%\end{theorem}


\textbf{Lemma}\ref{lem:dist} 
Fix a benchmark action $\base\in\points$.
If \eqref{eq:GOLD} is run with assumptions as above
and
we let $\breg_{\run} = (1/2) \norm{\state_{\run} - \base}^{2}$,
we have
\begin{equation}
\begin{split}
%(1/2) \norm{\state_{\run+1} - \base}^{2}
\breg_{\run+1}
	\leq \breg_{\run}
	&
		+ \step_{\run} \braket{\payv(\state_{\run})}{\state_{\run} - \base}
	\\
	&
		+ \step_{\run} \braket{\noise_{\head_{\run}+1}}{\state_{\run} - \base}
	\\
	&
		+ \step_{\run} \braket{\bias_{\head_{\run}}}{\state_{\run} - \base}
	\\
	&
		+ \tfrac{1}{2} \step_{\run}^{2} \norm{\hat\payv_{\run}}^{2}
\end{split}
\end{equation}
%\end{lemma}

\begin{proof}[Proof]
Since  $\est{\payv}_{\run}$ is a noisy estimate of $ \payv(\state_{\head_{\run}})$, we can decompose it as
\begin{equation}
\label{IV}
\est{\payv}_{\run} = \payv(\state_{\head_{\run}}) +\noise_{\head_{\run}+1} + \bias_{\head_{\run}},
\end{equation}
where:
\begin{enumerate}
\item
the noise process $\noise_{\head_{\run}+1} = \est{\payv}_{\run} -  \exof{\est{\payv}_{\run}\given \filter_{\run}}$ is a martingale difference sequence
\item
$\bias_{\head_{\run}} = \exof{\est\payv_{\run} \given \filter_{\run}} - \payv(\state_{\head_{\run}})$ denotes the systematic (non-zero-mean) error of the estimator $\est\payv_{\run}$ relative to the gradient of the dequeued state $\state_{\run}$.
\end{enumerate}
Where the filtration$\filter_{\run}$ contains all the random variables that have been realized at the beginning of the $\run$-th iteration of the algorithm;
more precisely, we let
\begin{equation}
\label{eq:filter}
\filter_{\run}
	= \sigma(
		\varnothing,
		\state_{\start},
%		\est\pay_{\head_{\start}},\unitvar_{\start},\head_{\start},\state_{2},
		\dotsc,
		\est\pay_{\head_{\run-1}},\unitvar_{\run-1},\state_{\run})
%	= \{\est{\pay}_{\head_\runalt}, \est{\state}_\runalt, \head_\runalt\}_{\runalt< \run} \union \{\state_\runalt\}_{\runalt\leq\run}
\end{equation}
with the convention $\est\pay_{\infty} = 0$, $\unitvar_{\infty} = 0$ if $\head_{\run} = \infty$.
We note for posterity that $\noise_{\head_{\run}}$ is a martingale difference sequence relative to $\filter_{\run}$, \ie $\exof{\noise_{\head_{\run}+1} \given \filter_{\run}} = 0$.
We also note here that, when the pool is empty, there is no update so $\state_{\run+1} = \state_{\run}$.
Then, for any $\base\in\points$ and for all $\run=\running\nRuns$ such that an update occurs, we have

\begin{align}
\label{eq:start}
\frac{1}{2}\norm{\base-\state_{\run+1}}^2& = \frac{1}{2}\norm{\base-\Eucl(\state_{\run} + \step_\run\est{\payv}_\run)}^2
	\notag\\
	&\leq \frac{1}{2}\norm{\base-\state_{\run}}^2+ \step_\run \braket{\est{\payv}_\run}{\state_\run - \base} + \frac{\step_\run^2}{2}\norm{\est{\payv}_\run}^2\\
	&=\frac{1}{2}\norm{\base-\state_{\run}}^2 + \step_\run \braket{\payv(\state_{\head_{\run}}) +\noise_{\head_{\run}+1} + \bias_{\head_{\run}} }{\state_\run - \base} + \frac{\step_\run^2}{2}\norm{\est{\payv}_\run}^2 \notag\\
	&= \frac{1}{2}\norm{\base-\state_{\run}}^2 +  \step_\run\braket{\payv(\state_{\run})}{\state_{\run} - \base} + \step_{\run} \braket{\noise_{\head_{\run}+1}}{\state_{\run} - \base}+ \step_{\run} \braket{\bias_{\head_{\run}}}{\state_{\run} - \base}+ \tfrac{1}{2} \step_{\run}^{2} \norm{\hat\payv_{\run}}^{2}\notag
\end{align}
\normalsize
\end{proof}

We can now prove the \cref{thm:regret}.

\textbf{Theorem} \ref{thm:regret}
Suppose that an agent is running \eqref{eq:GOLD} with step-size and sampling radius sequences of the form
$\step_{\run} = \step/\run^{c}$ and $\mix_{\run} = \mix/\run^{b}$ for some $\step,\mix > 0$ and
$b = \min\{1/4,1/3-\alpha/3\}$,
$c = \max\{3/4,2/3+\alpha/3\}$.
%$b,c$ defined below.
Then, the agent enjoys the mean regret bound
%\PM{Could you please check that this still makes sense?}
\begin{equation}
\label{eq:reg-bound}
\overline\reg(\nRuns)
	= \tilde\bigoh\parens[\big]{\nRuns^{3/4} + \nRuns^{2/3 + \alpha/3}}.
%	= \bigoh\parens[\big]{\nRuns^{\max\{3/4,2/3+\alpha/3\}}}
\end{equation}
%with $b = \min\{1/4,1/3-\alpha/3\}$ and $c = \max\{3/4,2/3+\alpha/3\}$.
%\end{theorem}


\begin{proof}[Proof]

Starting by the result of \cref{lem:dist}, for any $\point \in\points$ and for all $\run=\running\nRuns$ such that an update occurs, we have:

\begin{equation}
\step_\run\braket{\payv(\state_{\run})}{\point -\state_{\run} } 
	\leq \frac{1}{2}\norm{\point-\state_{\run}}^2 - \frac{1}{2}\norm{\point-\state_{\run+1}}^2 +\step_\run \sum_{\runalt=\head_{\run}}^{\run-1} \braket{\payv(\state_{\runalt}) - \payv(\state_{\runalt +1})}{\state_{\run} - \point}+ \step_\run\snoise_{\head_{\run}+1} + \step_{\run}r_{\head_{\run}} + \frac{\step_{\run}^2}{2}\norm{\est{\payv}_{\run}}^2
		%&\leq \breg_{{\run}} +\step_\run \sum_{\runalt=\head_{\run}}^{\run-1} \braket{\payv(\state_{\runalt}) - \payv(\state_{\runalt +1})}{\state_{\run} - \eq} + \step_\run\snoise_{\head_{\run}+1} + \step_{\run}r_{\head_{\run}} + \frac{\step_{\run}^2}{2K}\norm{\est{\payv}_{\run}}^2
\end{equation}

where we set $\snoise_{\head_{\run}+1} = \braket{\noise_{\head_{\run}+1}}{\state_{\run} - \point}$, $r_{\head_{\run}}= \braket{\bias_{\head_{\run}}}{\state_{\run} - \point}$.
Thus conditioning on $\filter_{\run}$ and taking expectations, we get 

\begin{equation}
\begin{split}
\step_\run\exof{\braket{\payv(\state_{\run})}{\point -\state_{\run} }\given \filter_{\run}} &\leq \frac{1}{2}\norm{\point-\state_{\run}}^2 - \frac{1}{2}\exof{\norm{\point-\state_{\run+1}}^2\given \filter_{\run}} +\step_{\run} \exof{ \sum_{\runalt=\head_{\run}}^{\run-1} \braket{\payv(\state_{\runalt}) - \payv(\state_{\runalt +1})}{\state_{\run} - \point}\given\filter_{\run}}\\
							&\qquad + \step_{\run} \exof{\snoise_{\head_{\run}+1}\given \filter_{\run}}+ \step_{\run} \exof{r_{\head_\run} \given \filter_{\run}} + \frac{\step _{\run}^2}{2} \exof{\norm{\est{\payv}_\run}^2\given \filter_{\run}}\\
\step_\run\braket{\payv(\state_{\run})}{\point -\state_{\run} }&\leq\frac{1}{2}\norm{\point-\state_{\run}}^2 - \frac{1}{2}\exof{\norm{\point-\state_{\run+1}}^2\given \filter_{\run}}+ \step_{\run}\sum_{\runalt=\head_{\run}}^{\run-1} \braket{\payv(\state_{\runalt}) - \payv(\state_{\runalt +1})}{\state_{\run} - \point}\\
&\qquad+ \step_{\run} \exof{r_{\head_\run} \given \filter_{\run} } + \frac{V^2}{2}\frac{\step_{\run}^2}{\mix_{\head_{\run}}^2}
\end{split}
\end{equation}
where we set $V^2 = \sum_\play \vdim^2 \max\limits_{\point \in \points}\abs{\pay_\play(\point)}^2$ and we used the fact that $\state_\runalt$ is $\filter_{\run}$-measurable for $\runalt\leq \run$, so $\exof{\snoise_{\head_{\run}+1}\given \filter_{\run}}  = \braket{\exof{\noise_{\head_{\run}+1}\given\filter_{\run}}}{\state_{\run} - \point} =0$.

%where we used the fact that $\payv$ is Lipschitz continuous and $\norm{\payv^\mix-\payv}_{\infty} = \bigoh(\mix)$.
As $\payv$ is Lipschitz continuous, we have $\norm{\bias_{\run}}=\bigoh(\mix_\run)$.
\todo{how to we prove that on $b_t$}
This shows that there exists some $ B>0$ such that $r_{\head_{\run}}\leq B \mix_{\head_{\run}}$
We thus obtain:
\begin{align}
\label{eq:rec_breg}
\step_\run \braket{\payv(\state_{\run})}{\point -\state_{\run}} &\leq \frac{1}{2}\norm{\state_{\run} - \point}^2
		- \frac{1}{2}\exof{\norm{\state_{\run+1} - \point}^2\given \filter_\run} + \step_\run \sum_{\runalt=\head_{\run}}^{\run-1}
			\braket{\payv(\state_{\runalt}) - \payv(\state_{\runalt +1})}{\state_{\run} - \point}+ B\step_\run\mix_{\head_{\run}}
		+ \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2}
	\notag\\
	&\leq \frac{1}{2}\norm{\point-\state_{\run}}^2 -\frac{1}{2}\exof{\norm{\point-\state_{\run+1}}^2\given \filter_\run} + \step_\run\sum_{\runalt=\head_{\run}}^{\run-1} \norm{\payv(\state_{\runalt}) - \payv(\state_{\runalt +1})}\norm{\state_{\run} - \point} + B\step_\run\mix_{\head_{\run}} + \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2}
		\notag\\
		&\leq \frac{1}{2}\norm{\point-\state_{\run}}^2-\frac{1}{2}\exof{\norm{\point-\state_{\run+1}}^2\given \filter_\run} + \beta\step_\run\sum_{\runalt=\head_{\run}}^{\run-1} \norm{\state_{\runalt} - \state_{\runalt +1}}\norm{\state_{\run} - \point} + B\step_\run\mix_{\head_{\run}} + \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2}
		\notag\\
		&\leq \frac{1}{2}\norm{\point-\state_{\run}}^2-\frac{1}{2}\exof{\norm{\point-\state_{\run+1}}^2\given \filter_\run} +\beta \step_\run\sum_{\runalt=\head_{\run}}^{\run-1} \norm{\step_{\runalt} \est{\payv}_{\runalt}}\norm{\state_{\run} - \point} + B\step_\run\mix_{\head_{\run}} + \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2}
		\notag\\
		&\leq \frac{1}{2}\norm{\point-\state_{\run}}^2 -\frac{1}{2}\exof{\norm{\point-\state_{\run+1}}^2\given \filter_\run} +A \step_\run\sum_{\runalt=\head_{\run}}^{\run-1}\frac{\step_{\runalt}}{\mix_{\runalt}} + B\step_\run\mix_{\head_{\run}} + \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2}
\end{align}
where $A$ is a positive constant depending on  $\max\limits_{\point \in \points}\abs{\pay_\play(\point)}$ and $\max\limits_{\point \in \points}\abs{\payv_\play(\point)}$.

Using the concavity of $\pay$, we then obtain:

\begin{equation}
\pay(\point) - \pay(\state_{\run}) \leq \frac{\norm{\point-\state_{\run}}^2 -\exof{\norm{\point-\state_{\run+1}}^2\given \filter_{\run}}}{2\step_\run} + \frac{1}{\step_\run} \left(A \step_\run\sum_{\runalt=\head_{\run}}^{\run-1}\frac{\step_{\runalt}}{\mix_{\runalt}}+ B\step_\run\mix_{\head_{\run}} + \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2}\right)
\end{equation}
\normalsize

Then, using the fact that $\gamma_{\run}$ is decreasing and the convergence of series shown in \cref{lem:3sums}, a summation of the above yields:
\begin{equation}
\begin{split}
\sum_{\run=1}^{\nRuns} \one_{\pool_\run\neq\varnothing} (\pay(\point) - \pay(\state_{\run})) &\leq \sum_{\run=1}^{\nRuns} \frac{\norm{\point-\state_{\run}}^2 -\exof{\norm{\point-\state_{\run+1}}^2\given \filter_{\run}}}{2\step_\run}+ \frac{1}{\step_\nRuns}\sum_{\run=1}^{\nRuns}\one_{\pool_\run\neq\varnothing}\left(A \step_\run\sum_{\runalt=\head_{\run}}^{\run-1}\frac{\step_{\runalt}}{\mix_{\runalt}}+ B\step_\run\mix_{\head_{\run}} + \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2}\right)\\
	& = \sum_{\run=1}^{\nRuns}\frac{\norm{\point-\state_{\run}}^2 -\exof{\norm{\point-\state_{\run+1}}^2\given \filter_{\run}}}{2\step_\run} + \tilde\bigoh(\frac{1}{\step_\nRuns})\\
	&=\frac{\norm{\point-\state_{1}}^2}{2\step_1} -\frac{\exof{\norm{\point-\state_{\run+1}}^2\given \filter_{\nRuns}}}{2\step_{\nRuns}} +  \sum_{\run=2}^{\nRuns} (\frac{\norm{\point-\state_{\run}}^2}{2\step_\run} -\frac{\exof{\norm{\point-\state_{\run}}^2\given \filter_{\run-1}}}{2\step_{\run-1}} )+ \tilde\bigoh(\frac{1}{\step_\nRuns})\\
\end{split}
\end{equation}
\normalsize
Where the notation  $\tilde\bigoh(\frac{1}{\step_\nRuns})$ accounts for the potential $log(\nRuns)$ factor in the case where one of the conditions of \cref{lem:3sums} is an equality.
Finally, by the law of total expectation, we get:
\begin{equation}
\begin{split}
\exof{\sum_{\run=1}^{\nRuns}\one_{\pool_\run\neq\varnothing} (\pay(\point) - \pay(\state_{\run}))} &\leq \frac{\exof{\norm{\point-\state_{1}}^2}}{2\step_1} -\frac{\exof{\norm{\point-\state_{\nRuns+1}}^2}}{2\step_{\nRuns}}+ \sum_{\run=2}^{\nRuns}(\frac{\exof{\norm{\point-\state_{\run}}^2}}{2\step_\run} -\frac{\exof{\norm{\point-\state_{\run}}^2}}{2\step_{\run-1}} )+ \tilde\bigoh(\frac{1}{\step_\nRuns})\\
&\leq \frac{1}{2}\diam(\points)^2 \sum_{\run=2}^{\nRuns}(\frac{1}{\step_\run} -\frac{1}{\step_{\run-1}} )+ \tilde\bigoh(\frac{1}{\step_\nRuns})\\
&= \frac{\diam(\points)^2}{2\step_\nRuns} - \frac{\diam(\points)^2}{2\step_1} + \tilde\bigoh(\frac{1}{\step_\nRuns})\\
&=\tilde\bigoh(\frac{1}{\step_\nRuns})
\end{split}
\end{equation}
\normalsize

Recall now that the number of step with no updates is $o(\nRuns^\alpha)$ by \cref{lemma:delayedfeedback,lemma:delay}.
We thus conclude that:
\begin{equation}
\exof{\sum_{\run=1}^{\nRuns} (\pay(\point) -\pay(\state_{\run}))} = \tilde\bigoh(\frac{1}{\step_\nRuns} + \nRuns^\alpha) = \tilde\bigoh(\nRuns^c + \nRuns^\alpha)
\end{equation}
\normalsize

Using \cref{fig:b_and_c} as a visual aid, we see that the smallest admissible value of $c$ is $\frac{3}{4}$ if $\alpha\leq\frac{1}{4}$, or $\frac{2}{3}+\frac{\alpha}{3}$ otherwise \textendash\ \ie the intersection of the lines $b=2c-1-\alpha$ and $b=1-c$.
In addition, $c\geq\frac{2}{3}+\frac{\alpha}{3}>\alpha$ because $\alpha<1$.
Therefore, by choosing $c=\max(\frac{3}{4},\frac{2}{3}+\frac{\alpha}{3})$  and $b=\min(\frac{1}{4},\frac{1}{3}-\frac{\alpha}{3})$ to minimize the regret, we obtain
\begin{equation}
\exof*{\sum_{\run=1}^{\nRuns} (\pay(\point) -\pay(\state_{\run}))} = \tilde\bigoh(\nRuns^c ) = \tilde\bigoh(\nRuns^{\max(\frac{3}{4},\frac{2}{3}+\frac{\alpha}{3})})
\end{equation}
\normalsize
Consequently, the $\tilde\bigoh(\nRuns^\frac{3}{4})$ bandit bound is achieved for $c=\frac{3}{4}$, $b=\frac{1}{4}$ and $\alpha\leq\frac{1}{4}$.
\end{proof}


\section{Convergence to equilibrium}
In this section we prove \cref{thm:Nash} on the convergence to Nash equilibrium.
For organisational purposes, we divide the proof in two parts:
We first start by showing that the distance between $\state_{\run}$ and the game's (necessarily unique) \acl{NE} converges to a finit limit value;
subsequently, we extract a subsequence of the sequence of actions that converges to said equilibrium.
With these two results at hand, the theorem follows trivially (as the limit value of the distance must, necessarily, be $0$).

\begin{proposition}
\label{breg_conv}
Let $\eq$ be a Nash equilibrium of $\game$. Then, with assumptions as in \cref{thm:Nash}, the distance  $\norm{\eq-\state_\run}^2$ converges (a.s.) to a finite random variable $D_\infty$.
\end{proposition}


\begin{proof}
Let $\eq$ denote the game's (unique) \acl{NE};
then, by \eqref{eq:DSC}, we have:
\begin{equation}
\braket{\payv(\point)}{ \point - \sol} \leq 0 \qquad \forall \point \in \points, \point\neq\sol
\end{equation}
\normalsize
with equality if and only if $\point = \sol$.

To proceed, \cref{eq:rec_breg} in the proof of the no-regret bound of \cref{thm:regret} in the previous section yields
\begin{equation}
\frac{1}{2}\exof{\norm{\eq-\state_{\run+1}}^2\given \filter_{\run}} \leq \frac{1}{2}\norm{\eq-\state_{\run}}^2 +\one_{\pool_\run\neq\varnothing} \left(A \step_\run\sum_{\runalt=\head_{\run}}^{\run-1}\frac{\step_{\runalt}}{\mix_{\runalt}}+ B\step_\run\mix_{\head_{\run}} + \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2}\right)
\end{equation}
\normalsize
where $A$ is a positive constant depending on  $\max\limits_{\point \in \points}\abs{\pay_\play(\point)}$, $\max\limits_{\point \in \points}\abs{\payv_\play(\point)}$ and $B>0$.
Then, letting
\begin{equation}
R_\run
	= \frac{1}{2}\norm{\eq-\state_{\run}}^2 + \sum_{\runalt=\run}^\infty \one_{\pool_\runalt\neq\varnothing}[ A \step_{\runalt}\sum_{i=\head_{\runalt}}^{\runalt-1}\frac{\step_i}{\mix_i}+ B\step_{\runalt}\mix_{\head_{\runalt}} + \frac{V^2}{2} \frac{\step_{\runalt}^2}{\mix_{\head_{\runalt}}^2}]
\end{equation}
\normalsize
we get
\begin{equation}
\begin{split}
\exof{R_{\run+1}\given\filter_\run}&= \exof{\frac{1}{2}\norm{\eq-\state_{\run+1}}^2\given \filter_\run} +\sum_{\runalt=\run+1}^\infty \one_{\pool_\runalt\neq\varnothing} [ A \step_{\runalt}\sum_{i=\head_{\runalt}}^{\runalt-1}\frac{\step_i}{\mix_i}+ B\step_{\runalt}\mix_{\head_{\runalt}} + \frac{V^2}{2} \frac{\step_{\runalt}^2}{\mix_{\head_{\runalt}}^2}] \\
					&\leq \frac{1}{2}\norm{\eq-\state_{\run}}^2 +\one_{\pool_{\run+1}\neq\varnothing} [A \step_\run\sum_{\runalt=\head_{\run}}^{\run-1}\frac{\step_{\runalt}}{\mix_{\runalt}}+ B\step_\run\mix_{\head_{\run}} + \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2} ]+\sum_{\runalt=\run+1}^\infty \one_{\pool_\runalt\neq\varnothing} [ A \step_{\runalt}\sum_{i=\head_{\runalt}}^{\runalt-1}\frac{\step_i}{\mix_i}+ B\step_{\runalt}\mix_{\head_{\runalt}} + \frac{V^2}{2} \frac{\step_{\runalt}^2}{\mix_{\head_{\runalt}}^2}] \\
					&= \frac{1}{2}\norm{\eq-\state_{\run}}^2 + \sum_{\runalt=\run}^\infty \one_{\pool_\runalt\neq\varnothing} [ A \step_{\runalt}\sum_{i=\head_{\runalt}}^{\runalt-1}\frac{\step_i}{\mix_i}+ B\step_{\runalt}\mix_{\head_{\runalt}} + \frac{V^2}{2} \frac{\step_{\runalt}^2}{\mix_{\head_{\runalt}}^2}]\\
					&=R_\run,
\end{split}
\end{equation}
\normalsize

i.e, $R_\run$ is an $\filter_\run$-adapted super martingale. Since the series $\sum_{\runalt=\run}^\infty \step_{\runalt}\sum_{i=\head_{\runalt}}^{\runalt-1}\frac{\step_i}{\mix_i}$, $ \sum_{\runalt=\run}^\infty\step_{\runalt}\mix_{\head_{\runalt}}$ and $\sum_{\runalt=\run}^\infty \frac{\step_{\runalt}^2}{\mix_{\head_{\runalt}}^2}$ converge to a finite number,
the series $\sum_{\runalt=\run}^\infty  \one_{\pool_\runalt\neq\varnothing} \step_{\runalt}\sum_{i=\head_{\runalt}}^{\runalt-1}\frac{\step_i}{\mix_i}$, $ \sum_{\runalt=\run}^\infty  \one_{\pool_\runalt\neq\varnothing}\step_{\runalt}\mix_{\head_{\runalt}}$ and $\sum_{\runalt=\run}^\infty  \one_{\pool_\runalt\neq\varnothing} \frac{\step_{\runalt}^2}{\mix_{\head_{\runalt}}^2}$ also converge because all terms are positive and it follows that
\begin{equation}
\begin{split}
\ex[R_\run] & = \ex[\exof{R_\run \given \filter_{\run-1}}]\\
		&\leq \ex[R_{\run-1}]\leq \cdots \leq \ex[R_1]\\
		&\leq \ex[\frac{1}{2}\norm{\eq-\state_{1}}^2]  +  \sum_{\runalt=1}^\infty  \one_{\pool_\runalt\neq\varnothing}[ A \step_\run\sum_{\runalt=\head_{\run}}^{\run-1}\frac{\step_{\runalt}}{\mix_{\runalt}}+ B\step_\run\mix_{\head_{\run}} + \frac{V^2}{2} \frac{\step_\run^2}{\mix_{\head_{\run}}^2}]\\
		&\leq \infty
\end{split}
\end{equation}
\normalsize
i.e, $R_\run$ is uniformly bounded in $L^1$. Thus, using Doob's convergence theorem for supermartingales \citep{HH80}, it follows that $R_\run$ converges (a.s) to some finite random variable $R_\infty$. In turn, it follows that $\norm{\eq-\state_{\run}}^2$ converges (a.s) to some random variable $D_\infty$, as claimed.
\end{proof}

\begin{proposition}
\label{subseq_conv}
Suppose that assumptions of \cref{thm:Nash}hold. Then, there exists a subsequence $\state_{\run_\runalt}$ of \eqref{eq:GOLD} which converges to the game's \textpar{necessarily unique} \acl{NE} with probability $1$.
\end{proposition}


\begin{proof}
%Under the stated assumptions, it is straightforward to see that the set of \aclp{NE} of the game is closed.
%We begin by observing that the set $\sols$ of Nash equilibria of $\game$ is closed.
%Indeed, let $\sol_\run, \run = 1,2,\ldots,$ be a sequence of Nash equilibria converging to some limit point $\sol\in\points$; to show that $\sols$ is closed, it suffices to show that $\sol \in \sols$. However, since Nash equlibria of $\game$ satisfy the variational characterisation \ref{}, we also have $\braket{\payv(\point)}{ \point- \sol_\run} \leq 0$ for all $\point \in \points$.
%Hence, with $\sol_\run \to \sol$ as $\run \to \infty$, it follows that
%\begin{equation}
%\braket{\payv(\point)}{ \point - \sol} = \lim\limits_{\run \to \infty} \braket{\payv(\point)}{ \point - \sol_\run} \leq 0 \qquad \forall \point \in \points
%\end{equation}
%i.e., $\sol$ satisfies \eqref{}. Since $\game$ is monotone, we conclude that $\sol$ is a Nash equilibrium, as claimed.
Suppose ad absurdum that, with positive probability, the sequence $\state_\run$ generated by \eqref{eq:GOLD} does not admit $\eq$ as a limit point.
Conditioning on this event, there exists a (nonempty) compact set $\cvx \subset \points$ such that $\eq\notin\cvx$ and $\state_\run \in \cvx$ for all sufficiently large $\run$.
Therefore, by the continuity of $\payv$, there exists some $c>0$ such that
\begin{equation}
\label{eq:cborn}
\braket{\payv(\point)}{\point - \sol} \leq -c \qquad \forall \point \in \cvx.
\end{equation}

To proceed, if we telescope \eqref{eq:start} and use \eqref{IV}, we get
\begin{equation}
\begin{split}
\frac{1}{2}\norm{\sol-\state_{\run+1}}^2&\leq \frac{1}{2}\norm{\eq-\state_{1}}^2+ \sum_{\run=1}^{\nRuns}\step_\run \one_{\pool_\run\neq\varnothing}\braket{\payv(\state_\run)}{\state_\run - \eq} \\
&+ \sum_{\run=1}^{\nRuns}\step_\run \one_{\pool_\run\neq\varnothing}\sum_{\runalt=\head_{\run}}^{\run-1} \braket{\payv(\state_{\runalt}) - \payv(\state_{\runalt +1})}{\state_{\run} - \eq} \\
&+ \sum_{\run=1}^{\nRuns}\step_\run\one_{\pool_\run\neq\varnothing}\snoise_{\head_{\run}+1} + \sum_{\run=1}^{\nRuns}\step_{\run}\one_{\pool_\run\neq\varnothing}r_{\head_{\run}} \\
&+ \sum_{\run=1}^{\nRuns}\one_{\pool_\run\neq\varnothing}\frac{\step_{\run}^2}{2}\norm{\est{\payv}_{\run}}^2\\
\end{split}
\end{equation}
\normalsize
where as in the proof of Theorem \ref{breg_conv} we set $\snoise_{\head_{\run}+1} = \braket{\noise_{\head_{\run}+1}}{\state_{\run} - \eq}$, $r_{\head_{\run}}= \braket{\bias_{\head_{\run}}}{\state_{\run} - \eq}$.
Subsequently, letting $\nu_\nRuns =\sum_{\run=1}^{\nRuns}\step_\run$ and using \eqref{eq:cborn}, we obtain
\begin{equation}
\begin{split}
\frac{1}{2}\norm{\sol-\state_{\run+1}}^2&\leq \frac{1}{2}\norm{\eq-\state_{1}}^2 - \nu_\nRuns c + \nu_\nRuns \bigg[ \frac{\sum_{\run=1}^{\nRuns}\step_\run \one_{\pool_\run\neq\varnothing}\sum_{\runalt=\head_{\run}}^{\run-1} \braket{\payv(\state_{\runalt}) - \payv(\state_{\runalt +1})}{\state_{\run} - \eq}}{\nu_\nRuns} \\
& \quad + \frac{\sum_{\run=1}^{\nRuns}\step_\run\one_{\pool_\run\neq\varnothing}\snoise_{\head_{\run}+1}}{\nu_\nRuns} + \frac{\sum_{\run=1}^{\nRuns}\step_{\run}\one_{\pool_\run\neq\varnothing}r_{\head_{\run}}}{\nu_\nRuns} + \frac{\sum_{\run=1}^{\nRuns}\one_{\pool_\run\neq\varnothing}\step_{\run}^2\norm{\est{\payv}_{\run}}^2}{2\nu_\nRuns} \bigg]
\end{split}
\end{equation}
\normalsize

Since $\noise_{\head_\run}$ is a martingale difference sequence with respect to $\filter_\run$, we have $\exof{\snoise_{\head_\run+1} \given \filter_\run} =0$ (recall that $\state_\runalt$ is $\filter_\run$-measurable for all $\runalt\leq\run$ by construction). 
Moreover, also by construction, there exists some constant $\sigma >0$ such that
\begin{equation}
\norm{\noise_{\run+1}}^2\leq\frac{\sigma^2}{\mix_\run^2},
\end{equation}
\normalsize
and hence:
\begin{equation}
\begin{split}
\sum_{\run=1}^\infty \one_{\pool_\run\neq\varnothing}\step_\run^2 \exof{\snoise^2_{\head_\run+1}\given \filter_\run} &\leq \sum_{\run=1}^\infty \one_{\pool_\run\neq\varnothing}\step_\run^2 \norm{\state_\run-\sol}^2\exof{\norm{\noise_{\head_{\run+1}}}^2\given \filter_\run}\\
				&\leq \sum_{\run=1}^\infty \step_\run^2 \norm{\state_\run-\sol}^2\exof{\norm{\noise_{\head_{\run+1}}}^2\given \filter_\run}\\
				&\leq \diam(\points)^2 \sigma^2\sum_{\run=1}^{\infty} \frac{\step_\run^2}{\mix_\run^2}<\infty
\end{split}
\end{equation}
\normalsize
Therefore, by the law of large numbers for martingale difference sequences \cite{HH80}, we conclude that $\frac{\sum_{\run=1}^{\nRuns}\step_\run\one_{\pool_\run\neq\varnothing}\snoise_{\head_{\run}+1}}{\nu_\nRuns}$ converges to $0$ with probability $1$.

For the three other terms in brackets, we show in the proof of the regret bound that the sums in the respective numerators are finite.
Since $\lim\limits_{\run\to\infty}\nu_\run=\infty$, it then follows that the three terms converge to $0$.
%\AH{For the term in $\step^2$, the proof in your paper with david and Mario is more complicated, I don't why. Am I missing something ?}
We thus get$\frac{1}{2}\norm{\sol-\state_{\run+1}}^2\leq \frac{1}{2}\norm{\eq-\state_{1}}^2 - c \nu_\nRuns /2$ for $\nRuns$ large enough, and hence, $\norm{\eq-\state_{\run}}^2\to-\infty$, a contradiction.
Going back to our original assumption, this shows that at least one of the limit points of $\state_\run$ must lie in $\sols$, so our proof is complete

\end{proof}


We just showed in Proposition \ref{subseq_conv} that we can extract a subsequence of action such that $\norm{\state_{\run_\runalt} - \eq}\to0$.
Since we also showed that the distance between any Nash equilibrium and the sequence of actions converges to a finite number, we conclude that $\norm{\state_{\run} - \eq} \to 0$ and, hence, with $\mix_{\run}\to0$, we also get $\norm{\est\state_{\run} - \eq} \to 0$.
